An investigation of open cluster Melotte 72 using Gaia DR2

The estimation of the main parameters of star clusters is significant in astrophysical studies. The most important aspect of using the Gaia DR2 survey lies in the positions, parallax, and proper motions of cluster stars with homogeneous photometry that make the membership probability determine with high accuracy. In this respect, depending on Gaia DR2 database, an analysis of the open star cluster Melotte 72 is taking place here. It is located at a distance of 2345+/-108 pc with an age of 1.0+/-0.5 Gyr. In studying the radial density profile, the radius is found to be 5.0+/-0.15 arcmin. The reddening, the luminosity and mass functions, the total mass of the cluster, and the galactic geometrical distances (X_Sun, Y_Sun, Z_Sun), and the distance from the galactic center (R_g ) have been estimated as well. Our study has shown a dynamical relaxation behavior of Melotte 72.

==> melo72/table2.tex <==
\begin{center}
\begin{table*}[h]
\caption{The cluster members of Melotte 72.}
\label{TAB_COMP_ASTROPHOTO}
\centering
\begin{tabular}{cccccccccccc}
\hline
ID & RA    & DE    & Plx   & e\_{Plx} & pmRA     & e\_{pmRA} & pmDE     & e\_{pmDE} & Gmag  & BP-RP & MP \\
   & (deg) & (deg) & (mas) & (mas)   & (mas/yr) & (mas/yr) & (mas/yr) & (mas/yr) & (mag) & (mag) &    \\
\hline
  1 & 114.644 & -10.779 & 0.331 & 0.036 & -4.201 & 0.060 & 3.461 & 0.048 & 15.419 & 0.757 & 0.98\\
  2 & 114.614 & -10.774 & 0.421 & 0.081 & -4.081 & 0.131 & 3.468 & 0.098 & 16.812 & 0.887 & 0.98\\
  3 & 114.643 & -10.760 & 0.325 & 0.030 & -4.244 & 0.051 & 3.711 & 0.042 & 14.787 & 0.565 & 0.99\\
  4 & 114.647 & -10.774 & 0.309 & 0.033 & -4.348 & 0.057 & 3.606 & 0.044 & 15.182 & 0.614 & 0.96\\
  5 & 114.635 & -10.765 & 0.470 & 0.051 & -4.198 & 0.083 & 3.558 & 0.066 & 16.168 & 0.874 & 0.98\\
  6 & 114.631 & -10.768 & 0.574 & 0.164 & -3.808 & 0.267 & 3.595 & 0.204 & 18.213 & 1.172 & 0.94\\
  7 & 114.587 & -10.764 & 0.370 & 0.021 & -4.145 & 0.037 & 3.683 & 0.031 & 13.268 & 0.644 & 1.0\\
  8 & 114.590 & -10.753 & 0.648 & 0.159 & -3.602 & 0.250 & 3.460 & 0.193 & 18.068 & 1.174 & 0.87\\
  9 & 114.582 & -10.757 & 0.494 & 0.076 & -4.124 & 0.130 & 3.558 & 0.100 & 16.797 & 1.040 & 0.98\\
  10 & 114.597 & -10.757 & 0.383 & 0.053 & -4.262 & 0.084 & 3.667 & 0.066 & 16.086 & 0.812 & 0.99\\
  11 & 114.614 & -10.737 & 0.419 & 0.049 & -4.153 & 0.078 & 3.651 & 0.069 & 15.858 & 0.877 & 0.99\\
  12 & 114.608 & -10.750 & 0.288 & 0.095 & -4.313 & 0.155 & 3.763 & 0.121 & 17.023 & 0.952 & 0.95\\
  13 & 114.664 & -10.750 & 0.484 & 0.043 & -4.010 & 0.069 & 3.652 & 0.060 & 15.739 & 0.799 & 0.98\\
  14 & 114.661 & -10.757 & 0.441 & 0.060 & -4.132 & 0.096 & 3.744 & 0.082 & 16.380 & 0.965 & 0.99\\
  15 & 114.663 & -10.729 & 0.040 & 0.159 & -4.692 & 0.248 & 3.933 & 0.205 & 18.125 & 1.203 & 0.84\\
  16 & 114.687 & -10.737 & 0.384 & 0.086 & -3.981 & 0.135 & 3.671 & 0.118 & 17.091 & 0.987 & 0.98\\
  17 & 114.681 & -10.719 & 0.300 & 0.059 & -4.279 & 0.096 & 3.493 & 0.084 & 16.371 & 0.871 & 0.97\\
  18 & 114.675 & -10.741 & 0.215 & 0.089 & -4.097 & 0.144 & 3.710 & 0.121 & 17.230 & 1.136 & 0.96\\
  19 & 114.666 & -10.736 & 0.493 & 0.052 & -4.002 & 0.087 & 3.468 & 0.076 & 16.154 & 0.813 & 0.96\\
  20 & 114.627 & -10.728 & 0.367 & 0.052 & -4.124 & 0.083 & 3.758 & 0.068 & 16.187 & 0.837 & 0.99\\
  21 & 114.632 & -10.727 & 0.463 & 0.037 & -4.061 & 0.057 & 3.705 & 0.044 & 15.109 & 0.629 & 0.99\\
  22 & 114.625 & -10.741 & 0.410 & 0.042 & -4.118 & 0.074 & 3.702 & 0.059 & 15.733 & 0.763 & 0.99\\
  23 & 114.624 & -10.733 & 0.356 & 0.034 & -4.099 & 0.054 & 3.620 & 0.043 & 15.119 & 0.655 & 0.99\\
  24 & 114.617 & -10.729 & 0.590 & 0.112 & -4.112 & 0.183 & 3.852 & 0.151 & 17.298 & 1.034 & 0.92\\
  25 & 114.650 & -10.729 & 0.305 & 0.036 & -4.039 & 0.059 & 3.470 & 0.051 & 15.385 & 0.678 & 0.98\\
  26 & 114.632 & -10.736 & 0.377 & 0.027 & -4.215 & 0.046 & 3.646 & 0.037 & 14.643 & 0.659 & 0.99\\
  27 & 114.649 & -10.731 & 0.400 & 0.047 & -4.242 & 0.078 & 3.693 & 0.061 & 16.014 & 0.781 & 0.99\\
  28 & 114.644 & -10.720 & 0.278 & 0.050 & -4.245 & 0.082 & 3.654 & 0.066 & 16.083 & 0.784 & 0.97\\
  29 & 114.653 & -10.715 & 0.406 & 0.041 & -4.215 & 0.066 & 3.694 & 0.057 & 15.643 & 0.724 & 0.99\\
  30 & 114.671 & -10.712 & 0.385 & 0.033 & -4.220 & 0.058 & 3.773 & 0.051 & 12.798 & 1.278 & 0.99\\
  31 & 114.658 & -10.710 & 0.388 & 0.048 & -4.050 & 0.076 & 3.783 & 0.054 & 12.658 & 0.557 & 0.99\\
  32 & 114.644 & -10.706 & 0.387 & 0.034 & -4.102 & 0.054 & 3.684 & 0.047 & 12.516 & 1.294 & 1.0\\
  33 & 114.649 & -10.710 & 0.360 & 0.028 & -4.281 & 0.044 & 3.687 & 0.038 & 14.436 & 0.582 & 0.99\\
  34 & 114.634 & -10.713 & 0.373 & 0.031 & -4.209 & 0.050 & 3.737 & 0.042 & 14.902 & 0.641 & 0.99\\
  35 & 114.653 & -10.721 & 0.354 & 0.025 & -4.151 & 0.041 & 3.745 & 0.035 & 14.337 & 0.594 & 1.0\\
  36 & 114.642 & -10.709 & 0.425 & 0.120 & -4.644 & 0.185 & 3.690 & 0.152 & 17.619 & 1.219 & 0.89\\
  37 & 114.650 & -10.727 & 0.374 & 0.031 & -4.193 & 0.051 & 3.680 & 0.044 & 14.966 & 0.572 & 1.0\\
  38 & 114.579 & -10.749 & 0.465 & 0.110 & -3.828 & 0.174 & 3.455 & 0.142 & 17.488 & 1.044 & 0.93\\
  39 & 114.564 & -10.739 & 0.242 & 0.077 & -4.169 & 0.139 & 3.751 & 0.110 & 16.662 & 0.905 & 0.96\\
  40 & 114.557 & -10.750 & 0.347 & 0.048 & -3.966 & 0.079 & 3.638 & 0.062 & 15.957 & 0.856 & 0.99\\
  41 & 114.584 & -10.751 & 0.357 & 0.139 & -4.208 & 0.220 & 3.853 & 0.175 & 17.892 & 1.124 & 0.95\\
  42 & 114.577 & -10.742 & 0.505 & 0.193 & -3.899 & 0.302 & 3.166 & 0.233 & 18.414 & 1.316 & 0.89\\
  43 & 114.584 & -10.739 & 0.391 & 0.105 & -4.094 & 0.165 & 3.719 & 0.132 & 17.332 & 1.006 & 0.98\\
  44 & 114.602 & -10.725 & 0.268 & 0.047 & -4.268 & 0.075 & 3.716 & 0.060 & 15.907 & 0.773 & 0.96\\
  45 & 114.587 & -10.715 & 0.338 & 0.038 & -4.197 & 0.064 & 3.739 & 0.049 & 15.388 & 0.670 & 0.99\\
  46 & 114.600 & -10.731 & 0.364 & 0.041 & -4.301 & 0.067 & 3.781 & 0.054 & 15.613 & 0.714 & 0.96\\
  47 & 114.604 & -10.729 & 0.399 & 0.050 & -4.091 & 0.082 & 3.769 & 0.065 & 16.075 & 0.781 & 0.99\\
  48 & 114.589 & -10.733 & 0.335 & 0.061 & -4.447 & 0.097 & 3.638 & 0.076 & 16.336 & 0.968 & 0.94\\
  49 & 114.573 & -10.731 & 0.747 & 0.153 & -3.886 & 0.243 & 3.766 & 0.185 & 18.013 & 1.145 & 0.91\\
  50 & 114.562 & -10.731 & 0.420 & 0.078 & -3.996 & 0.134 & 3.769 & 0.099 & 16.919 & 0.972 & 0.98\\
  51 & 114.545 & -10.719 & 0.331 & 0.041 & -4.228 & 0.072 & 3.685 & 0.058 & 15.478 & 0.686 & 0.99\\
  52 & 114.561 & -10.701 & 0.282 & 0.109 & -4.387 & 0.184 & 3.533 & 0.145 & 17.494 & 1.052 & 0.96\\
  53 & 114.560 & -10.709 & 0.244 & 0.154 & -4.282 & 0.248 & 3.643 & 0.188 & 18.065 & 1.178 & 0.95\\
  54 & 114.568 & -10.709 & 0.367 & 0.034 & -4.102 & 0.056 & 3.498 & 0.043 & 15.114 & 0.726 & 0.99\\
  55 & 114.571 & -10.705 & 0.497 & 0.177 & -4.502 & 0.282 & 3.616 & 0.216 & 18.285 & 1.217 & 0.93\\
  56 & 114.551 & -10.708 & 0.111 & 0.172 & -4.076 & 0.276 & 3.466 & 0.208 & 18.250 & 1.429 & 0.95\\
  57 & 114.570 & -10.706 & 0.218 & 0.107 & -4.386 & 0.174 & 3.958 & 0.131 & 17.431 & 1.035 & 0.87\\
  58 & 114.618 & -10.701 & 0.474 & 0.102 & -4.082 & 0.170 & 3.755 & 0.142 & 17.400 & 1.168 & 0.97\\
  59 & 114.610 & -10.719 & 0.435 & 0.153 & -3.889 & 0.235 & 3.708 & 0.180 & 17.955 & 1.118 & 0.96\\
  60 & 114.609 & -10.717 & 0.426 & 0.056 & -4.279 & 0.099 & 3.599 & 0.075 & 16.195 & 0.813 & 0.98\\
\end{tabular}
\end{table*}
\end{center}

 \setcounter{table}{1}

\begin{table*} \caption{continued}
\begin{tabular}{cccccccccccc}
\hline
ID & RA    & DE    & Plx   & e\_{Plx} & pmRA     & e\_{pmRA} & pmDE     & e\_{pmDE} & Gmag  & BP-RP & MP \\
   & (deg) & (deg) & (mas) & (mas)   & (mas/yr) & (mas/yr) & (mas/yr) & (mas/yr) & (mag) & (mag) &    \\
\hline 
  61 & 114.623 & -10.709 & 0.387 & 0.130 & -4.419 & 0.202 & 3.881 & 0.159 & 17.719 & 1.066 & 0.91\\
  62 & 114.606 & -10.713 & 0.355 & 0.027 & -4.099 & 0.046 & 3.633 & 0.037 & 12.972 & 1.234 & 1.0\\
  63 & 114.618 & -10.720 & 0.363 & 0.020 & -3.956 & 0.033 & 3.719 & 0.026 & 13.337 & 0.631 & 0.99\\
  64 & 114.599 & -10.707 & 0.401 & 0.031 & -4.138 & 0.050 & 3.685 & 0.037 & 13.896 & 0.458 & 1.0\\
  65 & 114.605 & -10.710 & 0.427 & 0.026 & -4.094 & 0.045 & 3.736 & 0.036 & 14.253 & 0.487 & 0.99\\
  66 & 114.608 & -10.710 & 0.348 & 0.032 & -4.032 & 0.052 & 3.601 & 0.042 & 15.051 & 0.595 & 0.99\\
  67 & 114.617 & -10.716 & 0.350 & 0.047 & -4.232 & 0.076 & 3.537 & 0.061 & 16.008 & 0.772 & 0.98\\
  68 & 114.621 & -10.717 & 0.390 & 0.029 & -4.031 & 0.046 & 3.607 & 0.037 & 14.793 & 0.622 & 0.99\\
  69 & 114.613 & -10.712 & 0.599 & 0.080 & -4.406 & 0.132 & 4.276 & 0.105 & 15.969 & 0.923 & 0.78\\
  70 & 114.609 & -10.708 & 0.347 & 0.031 & -4.119 & 0.048 & 3.665 & 0.038 & 12.950 & 1.237 & 1.0\\
  71 & 114.608 & -10.698 & 0.382 & 0.029 & -4.061 & 0.049 & 3.586 & 0.039 & 14.754 & 0.534 & 0.99\\
  72 & 114.617 & -10.712 & 0.482 & 0.028 & -4.164 & 0.046 & 3.655 & 0.037 & 14.788 & 0.636 & 0.99\\
  73 & 114.621 & -10.712 & 0.387 & 0.144 & -4.066 & 0.231 & 3.530 & 0.180 & 18.001 & 1.271 & 0.97\\
  74 & 114.598 & -10.708 & 0.432 & 0.135 & -4.084 & 0.205 & 3.731 & 0.160 & 17.584 & 1.021 & 0.97\\
  75 & 114.613 & -10.698 & 0.410 & 0.047 & -3.944 & 0.072 & 3.790 & 0.052 & 15.434 & 0.679 & 0.98\\
  76 & 114.621 & -10.703 & 0.419 & 0.021 & -4.110 & 0.034 & 3.714 & 0.027 & 13.576 & 0.593 & 1.0\\
  77 & 114.615 & -10.709 & 0.372 & 0.020 & -4.143 & 0.032 & 3.732 & 0.026 & 13.354 & 0.480 & 1.0\\
  78 & 114.628 & -10.714 & 0.428 & 0.051 & -4.062 & 0.082 & 3.629 & 0.066 & 16.143 & 0.813 & 0.99\\
  79 & 114.606 & -10.700 & 0.347 & 0.030 & -4.116 & 0.047 & 3.619 & 0.035 & 13.415 & 0.280 & 0.99\\
  80 & 114.649 & -10.695 & 0.349 & 0.026 & -4.138 & 0.052 & 3.642 & 0.035 & 13.618 & 0.452 & 0.99\\
  81 & 114.622 & -10.683 & 0.544 & 0.144 & -4.169 & 0.221 & 3.721 & 0.173 & 17.929 & 1.095 & 0.95\\
  82 & 114.617 & -10.689 & 0.399 & 0.036 & -4.012 & 0.058 & 3.921 & 0.046 & 15.288 & 0.662 & 0.93\\
  83 & 114.615 & -10.691 & 0.281 & 0.037 & -4.053 & 0.061 & 3.679 & 0.049 & 15.443 & 0.685 & 0.98\\
  84 & 114.624 & -10.705 & 0.369 & 0.023 & -4.022 & 0.037 & 3.724 & 0.031 & 14.014 & 0.501 & 1.0\\
  85 & 114.624 & -10.695 & 0.340 & 0.058 & -4.214 & 0.093 & 3.498 & 0.068 & 16.182 & 0.805 & 0.98\\
  86 & 114.629 & -10.703 & 0.354 & 0.023 & -4.099 & 0.036 & 3.620 & 0.029 & 13.879 & 0.505 & 1.0\\
  87 & 114.626 & -10.703 & 0.328 & 0.163 & -4.224 & 0.254 & 3.991 & 0.198 & 18.206 & 1.425 & 0.92\\
  88 & 114.626 & -10.692 & 0.274 & 0.034 & -4.409 & 0.054 & 3.886 & 0.040 & 14.865 & 0.682 & 0.87\\
  89 & 114.648 & -10.693 & 0.302 & 0.032 & -4.234 & 0.059 & 3.729 & 0.044 & 12.959 & 1.261 & 0.98\\
  90 & 114.626 & -10.683 & 0.367 & 0.022 & -4.132 & 0.037 & 3.652 & 0.031 & 13.833 & 0.525 & 1.0\\
  91 & 114.646 & -10.697 & 0.388 & 0.096 & -4.394 & 0.162 & 3.857 & 0.142 & 17.291 & 0.963 & 0.91\\
  92 & 114.636 & -10.685 & 0.518 & 0.114 & -3.497 & 0.170 & 3.580 & 0.131 & 17.198 & 1.180 & 0.79\\
  93 & 114.641 & -10.688 & 0.394 & 0.030 & -4.252 & 0.051 & 3.644 & 0.045 & 14.873 & 0.587 & 0.99\\
  94 & 114.624 & -10.696 & 0.438 & 0.036 & -4.195 & 0.057 & 3.728 & 0.045 & 15.303 & 0.618 & 0.99\\
  95 & 114.629 & -10.695 & 0.309 & 0.022 & -4.317 & 0.036 & 3.676 & 0.029 & 13.958 & 0.590 & 0.97\\
  96 & 114.624 & -10.687 & 0.373 & 0.021 & -4.075 & 0.034 & 3.729 & 0.027 & 13.589 & 0.603 & 1.0\\
  97 & 114.617 & -10.696 & 0.395 & 0.067 & -4.179 & 0.106 & 3.673 & 0.077 & 16.400 & 0.843 & 0.99\\
  98 & 114.616 & -10.697 & 0.323 & 0.038 & -4.170 & 0.059 & 3.738 & 0.043 & 15.033 & 0.573 & 0.99\\
  99 & 114.619 & -10.689 & 0.305 & 0.075 & -4.362 & 0.116 & 4.003 & 0.092 & 16.784 & 0.953 & 0.86\\
  100 & 114.623 & -10.698 & 0.324 & 0.043 & -3.918 & 0.070 & 3.637 & 0.056 & 15.839 & 0.851 & 0.98\\
  101 & 114.627 & -10.698 & 0.372 & 0.026 & -4.145 & 0.041 & 3.657 & 0.032 & 14.324 & 0.464 & 1.0\\
  102 & 114.638 & -10.686 & 0.346 & 0.029 & -4.081 & 0.044 & 3.674 & 0.034 & 13.786 & 0.479 & 1.0\\
  103 & 114.591 & -10.704 & 0.409 & 0.029 & -4.276 & 0.049 & 3.749 & 0.038 & 14.672 & 0.591 & 0.98\\
  104 & 114.583 & -10.679 & 0.472 & 0.154 & -3.765 & 0.259 & 3.732 & 0.202 & 18.009 & 1.328 & 0.95\\
  105 & 114.578 & -10.688 & 0.374 & 0.050 & -4.259 & 0.080 & 3.788 & 0.062 & 16.055 & 0.797 & 0.97\\
  106 & 114.589 & -10.681 & 0.359 & 0.073 & -4.255 & 0.116 & 3.491 & 0.093 & 16.709 & 1.018 & 0.98\\
  107 & 114.592 & -10.682 & 0.417 & 0.063 & -4.038 & 0.100 & 3.789 & 0.080 & 16.549 & 0.982 & 0.98\\
  108 & 114.604 & -10.698 & 0.396 & 0.048 & -4.152 & 0.078 & 3.717 & 0.063 & 16.068 & 0.780 & 0.99\\
  109 & 114.590 & -10.687 & 0.586 & 0.125 & -4.193 & 0.208 & 3.615 & 0.155 & 17.757 & 1.049 & 0.96\\
  110 & 114.596 & -10.691 & 0.412 & 0.038 & -4.396 & 0.062 & 3.982 & 0.049 & 15.575 & 0.762 & 0.87\\
  111 & 114.594 & -10.694 & 0.277 & 0.051 & -4.244 & 0.086 & 3.571 & 0.067 & 16.167 & 0.821 & 0.96\\
  112 & 114.597 & -10.690 & 0.306 & 0.049 & -4.161 & 0.078 & 3.888 & 0.063 & 16.035 & 0.781 & 0.94\\
  113 & 114.601 & -10.690 & 0.654 & 0.198 & -4.219 & 0.298 & 3.644 & 0.245 & 18.395 & 1.283 & 0.94\\
  114 & 114.610 & -10.665 & 0.347 & 0.112 & -4.495 & 0.183 & 3.563 & 0.141 & 17.625 & 1.124 & 0.94\\
  115 & 114.606 & -10.685 & 0.297 & 0.048 & -4.423 & 0.078 & 3.589 & 0.062 & 16.062 & 0.791 & 0.95\\
  116 & 114.612 & -10.684 & 0.339 & 0.022 & -4.103 & 0.036 & 3.672 & 0.029 & 13.886 & 0.506 & 1.0\\
  117 & 114.602 & -10.676 & 0.312 & 0.057 & -4.110 & 0.102 & 3.660 & 0.089 & 16.293 & 0.834 & 0.99\\
  118 & 114.599 & -10.680 & 0.434 & 0.028 & -4.181 & 0.047 & 3.656 & 0.037 & 14.857 & 0.554 & 0.99\\
  119 & 114.620 & -10.676 & 0.371 & 0.078 & -4.266 & 0.127 & 3.793 & 0.100 & 16.993 & 0.940 & 0.96\\
  120 & 114.611 & -10.674 & 0.363 & 0.020 & -4.160 & 0.032 & 3.709 & 0.026 & 13.275 & 1.253 & 1.0\\
 \end{tabular}
 \end{table*}

  \setcounter{table}{1}

\begin{table*} \caption{continued}
\begin{tabular}{cccccccccccc}
\hline
ID & RA    & DE    & Plx   & e\_{Plx} & pmRA     & e\_{pmRA} & pmDE     & e\_{pmDE} & Gmag  & BP-RP & MP \\
   & (deg) & (deg) & (mas) & (mas)   & (mas/yr) & (mas/yr) & (mas/yr) & (mas/yr) & (mag) & (mag) &    \\
\hline 
  121 & 114.602 & -10.671 & 0.341 & 0.035 & -4.148 & 0.060 & 3.910 & 0.050 & 15.258 & 0.709 & 0.93\\
  122 & 114.590 & -10.674 & 0.400 & 0.136 & -4.046 & 0.220 & 3.625 & 0.176 & 17.861 & 1.087 & 0.97\\
  123 & 114.617 & -10.686 & 0.203 & 0.134 & -4.059 & 0.214 & 3.326 & 0.168 & 17.879 & 1.124 & 0.95\\
  124 & 114.588 & -10.674 & 0.340 & 0.023 & -4.153 & 0.041 & 3.653 & 0.032 & 13.705 & 0.502 & 0.99\\
  125 & 114.615 & -10.682 & 0.527 & 0.138 & -4.352 & 0.218 & 3.636 & 0.171 & 17.947 & 1.122 & 0.95\\
  126 & 114.616 & -10.683 & 0.329 & 0.086 & -4.199 & 0.137 & 3.378 & 0.107 & 17.100 & 0.921 & 0.97\\
  127 & 114.608 & -10.690 & 0.339 & 0.028 & -4.054 & 0.045 & 3.771 & 0.036 & 14.704 & 0.541 & 0.99\\
  128 & 114.602 & -10.685 & 0.301 & 0.089 & -4.242 & 0.139 & 3.961 & 0.118 & 17.121 & 0.952 & 0.91\\
  129 & 114.682 & -10.707 & 0.417 & 0.069 & -4.223 & 0.111 & 3.794 & 0.092 & 16.648 & 0.891 & 0.97\\
  130 & 114.671 & -10.689 & 0.369 & 0.060 & -4.055 & 0.097 & 3.703 & 0.081 & 16.359 & 0.859 & 0.99\\
  131 & 114.671 & -10.703 & 0.352 & 0.024 & -4.244 & 0.044 & 3.599 & 0.038 & 14.072 & 0.480 & 0.99\\
  132 & 114.672 & -10.708 & 0.236 & 0.138 & -4.218 & 0.237 & 3.652 & 0.202 & 17.900 & 1.215 & 0.96\\
  133 & 114.690 & -10.696 & 0.402 & 0.074 & -4.612 & 0.117 & 3.625 & 0.099 & 16.737 & 0.891 & 0.88\\
  134 & 114.682 & -10.692 & 0.494 & 0.064 & -4.255 & 0.102 & 3.820 & 0.085 & 16.476 & 0.861 & 0.93\\
  135 & 114.675 & -10.686 & 0.323 & 0.105 & -4.230 & 0.164 & 3.573 & 0.135 & 17.394 & 1.035 & 0.97\\
  136 & 114.681 & -10.670 & 0.165 & 0.147 & -4.486 & 0.232 & 3.834 & 0.190 & 17.967 & 1.142 & 0.9\\
  137 & 114.696 & -10.674 & 0.336 & 0.026 & -4.163 & 0.042 & 3.723 & 0.037 & 13.008 & 1.230 & 1.0\\
  138 & 114.687 & -10.666 & 0.283 & 0.127 & -4.205 & 0.199 & 3.914 & 0.162 & 17.716 & 1.070 & 0.93\\
  139 & 114.697 & -10.679 & 0.373 & 0.079 & -4.008 & 0.127 & 3.442 & 0.107 & 16.905 & 0.922 & 0.98\\
  140 & 114.694 & -10.685 & 0.422 & 0.069 & -4.063 & 0.107 & 3.571 & 0.091 & 16.534 & 0.856 & 0.99\\
  141 & 114.647 & -10.681 & 0.328 & 0.030 & -4.135 & 0.050 & 3.653 & 0.040 & 12.994 & 0.605 & 0.99\\
  142 & 114.638 & -10.678 & 0.364 & 0.025 & -4.086 & 0.040 & 3.663 & 0.034 & 13.961 & 0.551 & 1.0\\
  143 & 114.636 & -10.676 & 0.190 & 0.098 & -4.302 & 0.157 & 3.516 & 0.132 & 17.317 & 0.995 & 0.95\\
  144 & 114.636 & -10.674 & 0.263 & 0.095 & -4.151 & 0.149 & 3.612 & 0.128 & 17.093 & 1.126 & 0.97\\
  145 & 114.644 & -10.677 & 0.390 & 0.090 & -4.452 & 0.159 & 3.384 & 0.135 & 17.185 & 1.059 & 0.95\\
  146 & 114.686 & -10.654 & 0.404 & 0.031 & -4.174 & 0.050 & 3.628 & 0.043 & 14.391 & 0.489 & 0.99\\
  147 & 114.637 & -10.668 & 0.345 & 0.021 & -4.153 & 0.038 & 3.629 & 0.033 & 13.096 & 1.263 & 0.99\\
  148 & 114.631 & -10.673 & 0.356 & 0.021 & -4.049 & 0.034 & 3.698 & 0.029 & 13.127 & 1.275 & 1.0\\
  149 & 114.643 & -10.664 & 0.428 & 0.064 & -3.943 & 0.104 & 3.778 & 0.089 & 16.527 & 0.889 & 0.98\\
  150 & 114.626 & -10.641 & 0.427 & 0.033 & -4.300 & 0.054 & 3.683 & 0.045 & 15.021 & 0.598 & 0.97\\
  151 & 114.626 & -10.655 & 0.403 & 0.044 & -4.237 & 0.069 & 3.594 & 0.059 & 15.650 & 0.728 & 0.99\\
  152 & 114.642 & -10.639 & 0.248 & 0.191 & -3.819 & 0.287 & 3.494 & 0.227 & 18.256 & 1.097 & 0.94\\
  153 & 114.657 & -10.632 & 0.355 & 0.027 & -4.137 & 0.046 & 3.675 & 0.038 & 14.513 & 0.492 & 1.0\\
  154 & 114.663 & -10.636 & 0.536 & 0.072 & -4.255 & 0.114 & 3.746 & 0.099 & 16.676 & 0.871 & 0.94\\
  155 & 114.659 & -10.648 & 0.572 & 0.109 & -4.110 & 0.172 & 3.561 & 0.143 & 17.477 & 1.033 & 0.96\\
  156 & 114.544 & -10.691 & 0.306 & 0.054 & -4.188 & 0.092 & 3.582 & 0.070 & 16.197 & 0.834 & 0.98\\
  157 & 114.546 & -10.695 & 0.538 & 0.158 & -3.852 & 0.258 & 4.130 & 0.190 & 18.085 & 1.166 & 0.85\\
  158 & 114.579 & -10.669 & 0.327 & 0.185 & -4.115 & 0.294 & 3.540 & 0.226 & 18.300 & 1.407 & 0.96\\
  159 & 114.566 & -10.678 & 0.486 & 0.036 & -4.135 & 0.060 & 3.657 & 0.048 & 15.451 & 0.749 & 0.99\\
  160 & 114.571 & -10.680 & 0.492 & 0.045 & -4.242 & 0.074 & 3.899 & 0.057 & 15.762 & 0.926 & 0.88\\
  161 & 114.568 & -10.675 & 0.410 & 0.074 & -4.212 & 0.130 & 3.543 & 0.101 & 16.810 & 0.916 & 0.98\\
  162 & 114.571 & -10.688 & 0.495 & 0.199 & -4.306 & 0.327 & 3.228 & 0.248 & 18.469 & 1.277 & 0.94\\
  163 & 114.558 & -10.674 & 0.371 & 0.055 & -4.130 & 0.091 & 3.751 & 0.071 & 16.239 & 0.835 & 0.99\\
  164 & 114.591 & -10.648 & 0.420 & 0.139 & -4.066 & 0.216 & 3.781 & 0.173 & 17.913 & 1.218 & 0.96\\
  165 & 114.599 & -10.636 & 0.429 & 0.028 & -4.054 & 0.047 & 3.680 & 0.041 & 14.683 & 0.588 & 0.99\\
  166 & 114.596 & -10.643 & 0.315 & 0.063 & -4.087 & 0.102 & 3.672 & 0.080 & 16.529 & 0.967 & 0.99\\
  167 & 114.623 & -10.633 & 0.370 & 0.032 & -4.066 & 0.054 & 3.774 & 0.047 & 14.859 & 0.596 & 0.99\\
  168 & 114.630 & -10.624 & 0.363 & 0.036 & -4.216 & 0.065 & 3.580 & 0.055 & 15.420 & 0.664 & 0.99\\
 \end{tabular}
 \end{table*} 
%\end{landscape}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


